A Necessary Step toward Faithfulness: Measuring and Improving Consistency in Free-Text Explanations

Faithful free-text explanations are important to ensure transparency in high-stakes AI decision-making contexts, but they are challenging to generate by language models and assess by humans. In this paper, we present a measure for Prediction-EXplanation (PEX) consistency, by extending the concept of weight of evidence. This measure quantifies how much a free-text explanation supports or opposes a prediction, serving as an important aspect of explanation faithfulness. Our analysis reveals that more than 62% explanations generated by large language models lack this consistency. We show that applying direct preference optimization improves the consistency of generated explanations across three model families, with improvement ranging from 43.1% to 292.3%. Furthermore, we demonstrate that optimizing this consistency measure can improve explanation faithfulness by up to 9.7%.

==> sections/problem.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=0.9\textwidth]{figures/pipeline.pdf}
\caption{TODO}
\label{fig:pipeline}
\end{figure*}


\label{sec:sft}

Machine learning models can excel at tasks where human are not naturally good at, for example at distinguishing between genuine and fake hotel reviews \cite{ott2011finding}.
Generating faithful free-text explanations from the models have potential to convey reasoning patterns for black-box model's predictions.
We consider the problem of measuring explanation quality and generating faithful explanations using large language models.

Formally, a language model $\model$ takes a question $\question$ as input, 
and generates an answer $\answer$ as its output. 
Question $\question$ is formatted as: $\question=$ \textpr{Is this  review truthful or deceptive? Review: \{review\}}. The output $\answer$ is \textpr{Truthful} or \textpr{Deceptive}.

\paragraph{Supervised fine-tuning to improve prediction accuracy.}

Off-the-shelf language models, including LLaMA-2 and Mistra models, do not perform well on the task of distinguishing truthful reviews from deceptive reviews, with prediction accuracy close to random guessing. Therefore, we finetune the model on the training dataset using supervised finetuning training (SFT) to have better estimation of $\model(\answer \mid \question)$. This is achieved by using the maximum-likelihood estimation (MLE) objective:

\begin{equation}
\sum_{D} log \model(\answer \mid \question)
\end{equation}

where the training dataset $D$ consisting of samples in the form of $(\question, \answer)$. The models achieve prediction accuracy of 94\% on the validation set.


\paragraph{Prompting for free-text explanation.}

We use the finetuned model $\model$ to generate an explanation $\explanation$ autoregressively for its answer: $\model(\explanation \mid \prompt(\question, \answer))$. The explanation $\explanation = (e_1, e_2, ..., e_n)$ is a sequence of words, e.g., \textpr{No specific examples: The review does not provide specific examples of the poor service or quality of the hotel.}
If $\model$ predicts the answer $\answer$ as \textpr{Truthful}, the prompt $\prompt$ is formatted as:
$\prompt(\question, \textpr{Truthful})=$ \textpr{Is this review truthful or deceptive? Review: \{review\}. Answer: Truthful. Question: Can you explain the main reasons why the review is truthful?}
If $\model$ predicts the answer $\answer$ as \textpr{Deceptive}, the prompt $\prompt$ is formatted as:
$\prompt(\question, \textpr{Deceptive})=$ \textpr{Is this review truthful or deceptive? Review: \{review\}. Answer: Deceptive. Question: Can you explain the main reasons why the review is deceptive?}

We use one-shot example to prompt the model to generate explanation for its prediction. The explanation usually contains 2-3 rationales. The explanations in the one-shot example are generated by GPT-4 (detailed in \autoref{app:explanation_prompting}).


\paragraph{An illustrative example.}

We find that the explanations can be inconsistent in that similar explanations are generated support both predictions.
For example, a model explains why a review is truthful because of  \textpr{balanced tone: The review does not excessively criticize the hotel or use overly emotional language.} 
On the other hand, it explains why the same hotel review is deceptive because of \textpr{limited emotional range: A genuine review would often provide more context and emotions, whether positive or negative, to make the experience more relatable.} 
The explanation ``language is not very emotional'' is used to support both predictions, hence this explanation is not consistent.

